Hierarchical Federated Learning with Momentum Acceleration in Multi-Tier Networks

In this paper, we propose Hierarchical Federated Learning with Momentum Acceleration (HierMo), a three-tier worker-edge-cloud federated learning algorithm that applies momentum for training acceleration. Momentum is calculated and aggregated in the three tiers. We provide convergence analysis for HierMo, showing a convergence rate of O(1/T). In the analysis, we develop a new approach to characterize model aggregation, momentum aggregation, and their interactions. Based on this result, {we prove that HierMo achieves a tighter convergence upper bound compared with HierFAVG without momentum}. We also propose HierOPT, which optimizes the aggregation periods (worker-edge and edge-cloud aggregation periods) to minimize the loss given a limited training time.

==> 1app_equivalent_new.tex <==
\subsection{Equivalent updates}
We first use variable transformation by introducing $\boldsymbol{v}_{i,\ell}^t=\boldsymbol{y}_{i,\ell}^t-\boldsymbol{y}_{i,\ell}^{t-1}$  and $\boldsymbol{x}_{i,\ell}^{t-1}=\boldsymbol{y}_{i,\ell}^{t-1}+\gamma\boldsymbol{v}_{i,\ell}^{t-1}$ with $\boldsymbol{v}_{i,\ell}^0=\boldsymbol{0}$ for all $i,\ell$. Then the HierMo local NAG updates and edge aggregation can be equivalently written as
\begin{align}
\boldsymbol{v}_{i,\ell}^t &\gets \gamma\boldsymbol{v}_{i,\ell}^{t-1} - \eta\nabla F_{i,\ell}(\boldsymbol{x}_{i,\ell}^{t-1}),\label{eq:localVi}\\ 
\boldsymbol{x}_{i,\ell}^t 
 &\gets \boldsymbol{x}_{i,\ell}^{t-1} + \gamma\boldsymbol{v}_{i,\ell}^t - \eta\nabla F_{i,\ell}(\boldsymbol{x}_{i,\ell}^{t-1}).\label{eq:localWi}\\
\boldsymbol{v}_\ell^t &\gets \sum_{i=1}^{C_\ell}\frac{ D_{i,\ell}}{D_\ell} \boldsymbol{v}_{i,\ell}^t,\quad
\label{eq:globalW}
\boldsymbol{x}_\ell^t \gets \sum_{i=1}^{C_\ell}\frac{ D_{i,\ell}}{D_\ell} \boldsymbol{x}_{i,\ell}^t.
\end{align}
Similarly, the edge and cloud centralized update rules can be equivalently written as
\begin{align}
\boldsymbol{v}_{[k],\ell}^t \gets& \gamma\boldsymbol{v}_{[k],\ell}^{t-1} - \eta\nabla F_{\ell}(\boldsymbol{x}_{[k],\ell}^{t-1}),\nonumber\\ 
\boldsymbol{x}_{[k],\ell}^t 
 \gets& \boldsymbol{x}_{[k],\ell}^{t-1} + \gamma\boldsymbol{v}_{[k],\ell}^t - \eta\nabla F_{\ell}(\boldsymbol{x}_{[k],\ell}^{t-1})\label{eq:xkt_app}. \\
\boldsymbol{v}_{\{p\}}^t \gets& \gamma\boldsymbol{v}_{\{p\}}^{t-1} - \eta\nabla F(\boldsymbol{x}_{\{p\}}^{t-1}),\nonumber\\ 
\boldsymbol{x}_{\{p\}}^t 
 \gets& \boldsymbol{x}_{\{p\}}^{t-1} + \gamma\boldsymbol{v}_{\{p\}}^t - \eta\nabla F(\boldsymbol{x}_{\{p\}}^{t-1})\label{eq:xpt_app}. 
\end{align}
%And the aggregated value of $\boldsymbol{v}^t$ and $\boldsymbol{x}^t$ can be written as
%\begin{align}%\label{eq:globalV}
%\boldsymbol{v}^t \gets \sum_{i=1}^N\frac{ D_i}{D} \boldsymbol{v}_i^t,\quad
%\label{eq:globalW}
%\boldsymbol{x}^t \gets \sum_{i=1}^N\frac{ D_i}{D} \boldsymbol{x}_i^t.
%\end{align}
Now, we use \eqref{eq:localVi} - \eqref{eq:xpt_app} to conduct the convergence analysis.  
